A Multivariate Multilevel Longitudinal Functional Model for Repeatedly Observed Human Movement Data

Biomechanics and human movement research often involves measuring multiple kinematic or kinetic variables regularly throughout a movement, yielding data that present as smooth, multivariate, time-varying curves and are naturally amenable to functional data analysis. It is now increasingly common to record the same movement repeatedly for each individual, resulting in curves that are serially correlated and can be viewed as longitudinal functional data. We present a new approach for modelling multivariate multilevel longitudinal functional data, with application to kinematic data from recreational runners collected during a treadmill run. For each stride, the runners' hip, knee and ankle angles are modelled jointly as smooth multivariate functions that depend on subject-specific covariates. Longitudinally varying multivariate functional random effects are used to capture the dependence among adjacent strides and changes in the multivariate functions over the course of the treadmill run. A basis modelling approach is adopted to fit the model -- we represent each observation using a multivariate functional principal components basis and model the basis coefficients using scalar longitudinal mixed effects models. The predicted random effects are used to understand and visualise changes in the multivariate functional data over the course of the treadmill run. In our application, our method quantifies the effects of scalar covariates on the multivariate functional data, revealing a statistically significant effect of running speed at the hip, knee and ankle joints. Analysis of the predicted random effects reveals that individuals' kinematics are generally stable but certain individuals who exhibit strong changes during the run can also be identified. A simulation study is presented to demonstrate the efficacy of the proposed methodology under realistic data-generating scenarios.

==> main/related-long.tex <==
\section{Literature Review}


% \textbf{\textcite{hyndman_robust_2007}} proposed the following approach for forecasting univariate functional time series data, :
% \begin{enumerate}
%     \item Smooth each functional observation individually.
%     \item Apply robust FPCA to the full functional dataset (ignoring time-series dependence) to obtain FPC basis functions and scores.
%     \item Model each score separately using univariate (scalar) time series models.
%     \item Forecast future (in time-series time) versions of the scores using the fitted models.
%     \item Combine the forecasted scores and FPC basis functions and add them to give a forecast of the functional variable.
%     \item Use variance estimates from the FPC and smoothing steps to compute functional prediction intervals for the forecast.
% \end{enumerate}
% They justify, (similar to us) the modelling of each score spearately because they are uncorrelated
% \begin{quote}
%      \emph{``\dots this is a multivariate time series problem. However, because of the way the basis functions have been chosen, the coefficients are uncorrelated. Therefore it is likely that univariate methods will be adequate for forecasting each series. There may still be cross-correlations at non-zero lags, but these are likely to be small given the zero contemporaneous correlations"}
% \end{quote}


------------------------------------------------------------------------------------------------------------------

\textbf{\textcite{greven_longitudinal_2010}} \emph{functional principal component analysis} paper.

\textbf{Definition:} \emph{Data sets containing functions or images that are observed repeatedly over time (longitudinal functional data).}

Focus on describing the process dynamics over longitudinal time using FPCA.

\paragraph{Model}
$$Y_{ij}(d) = \underbrace{\eta(d, T_{ij}))}_{\text{mean surface}} + \underbrace{X_{i,0}(d)}_{\text{Functional RI}} + \underbrace{X_{i,0}(d)}_{\text{Functional RS}} T_{ij} + \underbrace{U_{ij}(d)}_{\text{Smooth error}} + \underbrace{\epsilon_{ij} (d)}_{\text{White noise}}$$.


------------------------------------------------------------------------------------------------------------------

\textbf{\textcite{park_longitudinal_2015}} \emph{longitudinal functional data analysis} paper.


\textbf{Definition:} Longitudinal functional data consist of \emph{functional observations (such as profiles or images) observed at several times for each subject of many.}


\paragraph{Literature Review}
They note that many methods applied to multilevel functional data (I'm assuming they mean e.g., \textcite{di_multilevel_2009, morris_wavelet-based_2006}) do not take into account the ``actual time" that the functional observation is observed, i.e., they assume exchangeability in time. They note that \textcite{greven_longitudinal_2010} only focuses on describing the process dynamics, rather than prediction of a full future trajectory. They note that \textcite{chen_modeling_2012} have an approach but is computationally demanding.

\paragraph{Model setup}
The model is
$$
Y_{ij} (s)
= 
\mu(s, T_{ij})
+
X_i (s, T_{ij})
+
\varepsilon_{ij} (s)
$$
where 
\begin{itemize}
    \item $\mu(s, T_{ij})$ is the smooth mean
    \item $X_i (s, T_{ij})$ is the smooth random deviation from the mean for subject $i$ at time $T_{ij}$
    \item $\varepsilon_{ij} (s)$ is the smooth random deviation specific to observation $ij$.
\end{itemize}
The model is constructed with a \emph{sparse longitudinal} and  \emph{dense functional} design in mind \emph{\color{red}(note difference to our scenario)}. The key point is that $X_i(t)$ is expanded on a longitudinal time-invariant basis
$$
X_i(s, T_{ij}) = \sum _{k \geq 1} \xi_{ik} (T_{ij}) \phi_k(s),
$$
i.e., \emph{all of the the variation/ trend in the $T$ direction is captured by the scores}. The time-invariant basis used is the \emph{``marginal"} or \emph{``pooled"} basis, which is just a standard FPCA of the centered data, ignoring the dependence in the $T$ direction. 

The scores $\xi_{ik}(T_{ij})$ for each longitudinal-time-invariant basis function $\phi_k (s)$ are treated as functions $\xi_{ik} (T)$ with an unknown covariance function $G_k (\cdot, \cdot)$. They suggest using a parametric basis/ covariance (as we are planning to do/ \textcite{lee_bayesian_2019} have done) is a ``viable" option:
\begin{quote}
    \emph{``One viable approach is to assume a parametric structure for $G_k(\cdot, \cdot)$ such as AR(1) or a random effects model framework; this is typically preferable when $m_i$ is very small and the longitudinal design is balanced. We discuss random effects model for estimating the longitudinal covariance in the data application. Here we consider a more flexible approach and estimate the covariance $G_k(\cdot, \cdot)$  nonparametrically, by employing FPCA techniques for sparse functional data (Yao et al., 2005)."}
\end{quote}
However, they instead treat them as ``truly" functional data and a second K-L representation (now in longitudinal time) is used $\xi_{ik}(T_{ij}) = \sum_{l=1}^{\infty} \zeta_{ikl} \psi_{kl}(T_{ij})$. This results in the following (truncated) model representation
$$
Y_{ij} (s)
= 
\mu(s, T_{ij})
+
\sum_{k=1}^K
\sum_{l=1}^{L_k}
\zeta_{ikl} \psi_{kl}(T_{ij}) \phi_k (s)
+
\varepsilon_{ij} (s),
$$
where $\varepsilon_{ij} (s) = \sum_{k=1}^{K} \epsilon_{ijk} \phi_k(s) + \varepsilon_{2,ij} (s)$. The two parts of the error term can roughly be viewed as: 1) the remainder of the scores that are uncorrelated across $T$ multiplied by their respective basis function and 2) the part of each functional observation that is uncorrelated across $s$.

% Note, for example, that the random slope and intercept model of \textcite{greven_longitudinal_2010} is a special case with $\xi_{ik}(T_{ij}) = \zeta_{0, ik} + \zeta_{0, ik} T_{ij}$. They also make connections with other models.

\paragraph{Model Estimation}
\begin{steps}[leftmargin=2cm]
  \item Estimate $\mu(s, T)$ using a bivariate smoother  \parencite[e.g., tensor-product splines][]{wood_generalized_2017}. 
  \item Estimate the longitudinal-time-invariant basis by calculating the raw covariance. Because the data are measured with error the smoothing of the raw covariance can be done while ignoring the diagonal elements \parencite{yao_functional_2005, di_multilevel_2009}
  \item Use a PACE-style algorithm to do FPCA of each of the longitudinal-time-varying scores from the last step \parencite{yao_functional_2005}. The only difference is that PACE is designed for when functional data are observed (with error), here it is estimated scores from the last step the are being treated as the observed functions.
  \item Combine estimated scores from \emph{Step 2} and the basis functions from \emph{Step 2} and \emph{Step 3} to reconstruct the full trajectory.
\end{steps}

\paragraph{Theoretical Properties}
Details omitted but consistency of all model components proved for (i) No error term, and (ii) functions measured with smooth error. 

\paragraph{Simulation study}

Overview of simulation setup:
\begin{itemize}
    \item \textbf{Mean function}: Simple parametric function $\mu(s, T) = 1 + 2s + 3T + 4sT$
    \item \textbf{Longitudinal-time-invariant basis functions}: $K = 2$  with $\phi_1(s)=1$ and $\phi_2(s)=\sqrt{2}sin(2 \pi s)$
    \item \textbf{Grids}: $s$ is observed at 101 equally-spaced points in $[0, 1]$; $T$ observed at $m_i$ points sampled from $41$ equally-spaced points on $[0, 1]$
    \item \textbf{Longitudinal Coefficients}: Three covariance structures considered
    \begin{enumerate}
        \item \emph{Non-parametric covariance}: $\xi_{ik}(T) = \zeta_{ik1} \psi_{k1}(T) + \zeta_{ik2} \psi_{k2}(T)$
        \item \emph{Random-effects model}: $\xi_{ik}(T) = b_{ik0} + b_{ik1}T$
        \item \emph{Exponential autocorrelation}: $cov\{\xi_{ik}(T), \xi_{ik}(T')\} = \lambda_k \rho_k^{| T - T' |}$
    \end{enumerate}
    \item \textbf{Errors}: From $\varepsilon_{ij}(s)= \epsilon_{ij1} \phi_1(s) + \epsilon_{ij2} \phi_2(s) + \varepsilon_{2, ij} (s)$.
    \item \textbf{Test set}: The test set is created by selecting 10 subjects and holding out their last functional observation. The training set is all remaining data (from the other $n-10$ subjects and the functions up until the last from the selected subjects).
    \item \textbf{Practicalities}:
    \begin{itemize}
        \item  50 basis functions for the mean (tensor product of 10 marginal basis functions in the $s$ direction and $5$ marginal basis functions in the $T$ direction). Smoothing parameters estimated by REML.
        \item Truncations of $K$ and $K_l$ such that $95\%$ of variance is explained.
    \end{itemize}

Highlights of simulation results:

\begin{itemize}
    \item Prediction accuracy, both in-sample and out-of-sample is dependent on the longitudinal correlation structure and is worst for the Exponential autocorrelation, I guess this makes sense, as there is no obvious ``trend" to capture to help prediction.
    \item They compare to a naive approach of just predicting a profile based on all the subjects averages. As expected, longitudinal model substantially outperforms the naive method. Naive predictions are also much worse in the for the nonparametric longitudinal covariance than for the random-effects or exponential autocrrelation models.
    \item Also compare method to \textcite{chen_modeling_2012} and show improved prediction and computation times.
\end{itemize}
\end{itemize}

\paragraph{Application}
\begin{itemize}
    \item Application is to the DTI data which was used previously in other studies \parencite{greven_longitudinal_2010, scheipl_functional_2015}.
    \item Objectives: 
    \begin{enumerate}
        \item Understand dynamic behaviour of the CCA-FA profile in MS patients over time.
        \item Accurate predictions of the CCA-FA profile of a patient at their \emph{next} visit.
    \end{enumerate}
    \item They normalise longitudinal time $T$ to start at $0$ for subject's first visit and scale it using the maximum value from the \emph{entire sample}, rather than the subject's maximum time. The claim that this improves interpret-ability.
    \item There are only a few large $T_{ij}$'s ($\approx 1$) so they avoid doing bivariate smoothing for $\mu(s, T)$. Instead they use $\mu(s, T_{ij}) = \mu_0(s) + \beta_T (s) T_{ij}$. After fitting and using a bootstrap of subjects, they find that $\beta_T (s) \approx 0$, so $\mu_0(s)$ is sufficient.
    \item Extract $K=10$ marginal eigenfunctions explain $95\%$ of the variance.
    \item They \textbf{don't do a second FPCA}, instead they choose a simpler random slope model for each score (so they actually don't use the proposed methodology).
    \item Out of sample prediction error -- the approach actually only marginally improves over the naive approach. It's interesting that the new approach and naive approach both greatly outperform \textcite{chen_modeling_2012} method.
    
\end{itemize}


------------------------------------------------------------------------------------------------------------------



\textbf{\textcite{lee_bayesian_2019}} \emph{Bayesain Semiparametric Functional Mixed Models for Serially Correlated Functional Data with Application to Glaucoma data} paper.

This paper extends the BayesFMM paper of \textcite{morris_comparison_2017} to serially correlated functions and smooth non-parametric effects of scalar covariates, we are only concerned with the former. Note that they have data that's correlated over a continuous that's not time (not technically longitudinal functional data, but the same structure):

\begin{quote}
    \emph{``There are relatively few that model serially correlated functions, for which functions are observed at multiple levels of some continuous variable for the same subject. Most commonly, the functions occur along a grid of time points, which could be called \emph{longitudinally correlated functional data}, but can also occur over other continuous variables such as IOP for our glaucoma data."}
\end{quote}


They also note that many existing approaches for LFDA just focus on modelling the longitudinal trends rather than joint estimation of fixed effects and random effects structure. 

\begin{quote}
    \emph{``There are a number of articles that focus on functional predictor regression (Goldsmith et al. 2012; Gertheiss et al. 2013; Kundu, Harezlak, and Randolph 2016; Islam, Staicu, and van Heugten 2016) or estimate multi-level principal components (Greven et al. 2010; Zipunnikov et al. 2011; Chen and Muller 2012; Li and Guan 2014; Zipunnikov et al. 2014; Park and Staicu 2015; Shou et al. 2015; Hasenstab et al. 2017) for serially correlated functions, but these articles do not deal directly with functional response regression, that is, do not regress the functions on covariates while accounting for this serial correlation in the error structure."}
\end{quote}



In methods, we focus on Section 3.2 \textbf{\emph{``Accommodating Serial Interfunctional Correlation via
Functional Growth Curves"}}

The \emph{functional growth curve model} is for the functional variable $Y$ that varies smoothly across a serial variable $p$ IOP is
$$
Y_{ip} (t) = m(p, t) + u_i (p, t) + E_{ip} (t),
$$
where $m(p, t)$  is the mean MPS for IOP level $p$ and scleral location $t$, $u_i(p, t)$ is a mean zero random effect for subject $i$ that represents a subject-specific growth curve in $p$ that is allowed to vary across scleral location $t$, and $E_{ip}(t)$ are residual error functions assumed to be independent and identically distributed mean zero Gaussians with covariance $\mathbf{S}$. 

Fit the model by finding a \emph{\textbf{suitable parametric basis}} for the serial effect $s$ and assume that
$$
m(p, t) = \sum_{d=0}^D B_d(t) G_d(p)
$$
and
$$
u_i(p, t) =  \sum_{d=0}^D U_{id} (t) G_d(p).
$$
They recommend using basis functions that are \emph{orthogonal} across $d$, that is $\int  G_d(p)  G_d'(p) \textrm{d}p = 0$ and avoid estimating cross covariance terms between $U_{id}(t)$ and $U_{id'}(t)$. This model is then easilty incorporated into the BayesFMM framework, because it just has $D+1$ fixed and random effects functions. Note the interfunctional correlations that are induced across $t$ and $p$ by the respective basis functions.

They use a model selection heuristic (which they admit is very ad hoc) to determine the best fixed and random effects structure, that is:
\begin{enumerate}
    \item Transform the functional data to the basis space, for each $Y_i (t)$, compute the coefficients $Y_{i1},\dots, Y_{iK}*$ and then compute an importance weight $w_k$ for each coefficient, based on $w_k = \sum_{i=1}^N (Y_{ik}^*)^2 /  \sum_{i=1}^N \sum_{k=1}^K  (Y_{ik}^*)^2$, with $w_k=1$ \emph{\color{purple} I think these could be PVE for us with FPCs}.
    \item Fit scalar LMM and compute adapted BIC (aBIC) scores for each basis coefficient $k$ and each candidate model $c$. Adapted BIC is used in place of normal BIC because they are interested in random effects predictions in their application (in the ``penalised splines as mixed models sense" for their smooth non-parametric fixed effects).
    \item Use a weighted voting scheme to rank models. Compute a probability weight $P_c$ for each model $M_c, \ c= 1, \dots, C$:
    $$
    P_c = \sum_{k=1}^K w_k I\{c=argmin_{c'}BIC_{c'k}\},
    $$
    where the indicator function indicates whether model $M_c$ was the best of basis coefficient $k$.
\end{enumerate}

\textbf{Application:} Again we only really focus on the serial correlation part.

\begin{itemize}
    \item For the IOP effect they also had a three-level model, they had eye (left or right) within subject. Candidate models were constant, linear, hyperbolic or non-parametric IOP effect at both levels (hyperbolic was determined as a candidate earlier by fitting models pointwise).
    \item Model selection procedure identified model with no subject effect at all (not even a random intercept), and a hyperbolic IOP random effect for eye.
    \item IOP model parameterised as parabola $Y = b_0 + b_1 p + b_2 p^{-1}$. Then transformed them to be orthogonalised (have made plot).
    \item Considered summary of age effect integrated over IOP, which they term the area under the MPS vs. IOP curve \emph{\color{purple} need to get my head around this}.
    \item They then look at the derivative of this with respect to age \emph{\color{purple} gives me ideas about us going something similar with BLUPs}.
\end{itemize}

Conclusion, they have some nice points on why it's useful to try and model the full dataset:
\begin{quote}
    \emph{``This raises the obvious question, “What is the advantage of fitting the entire functional model? Why not just compute the aggregated summaries and model those using standard tools?” The answer to this question is multi-faceted.

    First, if one only looked at specific aggregated summaries, they may miss insights that could have been gleaned from their data but were not captured by these summaries. For example, if only looking at the PP and MP regions, one may miss out on different MPS behavior in the inferior and nasal regions of the sclera, which may be important. By modeling the scleral function in its entirety, we are able to examine the entire domain to ensure we are not missing out on any insights, and then we can still produce inference for any desired aggregated summaries for ease of interpretation, as well. This concept is also relevant in other application areas where summaries are used because of the complexity and high dimensionality of the raw functional data. This approach of flexible modeling followed by inference on summary measures can capture the best of both worlds, analyzing the entire function yet producing inference for summary measures interpretable for the scientific subject area.
    
    Second, any aggregation draws arbitrary boundaries in the function space.MPS for scleral locations at the boundary of the PP and MP regions are highly correlated with each other, and yet PP and MP extracted summaries arbitrarily separate them from each other. The flexible functional modeling framework introduced in this articlemodels the entire functional space, yet captures and accounts for intrafunctional correlation through the chosen basis functions. This allows a smooth borrowing of strength from nearby locations, and if location-scale bases like wavelets are used, then this borrowing of strength can be adaptive, able to accommodate spatially heterogenous functions for which some functional regions are more correlated than others. In principle, accounting for this intrafunctional correlation leads to greater efficiency, as has been shown in various contexts.
    }
\end{quote}
